Geometry Optimization of Crystals by the Quasi-Independent Curvilinear Coordinate Approximation

The quasi-independent curvilinear coordinate approximation (QUICCA) method [K. N\'emeth and M. Challacombe, J. Chem. Phys. {\bf 121}, 2877, (2004)] is extended to the optimization of crystal structures. We demonstrate that QUICCA is valid under periodic boundary conditions, enabling simultaneous relaxation of the lattice and atomic coordinates, as illustrated by tight optimization of polyethylene, hexagonal boron-nitride, a (10,0) carbon-nanotube, hexagonal ice, quartz and sulfur at the $\Gamma$-point RPBE/STO-3G level of theory.

==> figs <==
set term postscript eps  enhanced color "Courrier" 28
set output "UREA_321G.eps"

set encoding iso_8859_1
set style line  1 lt 1 lw 10 pt 1 ps 1.5
set boxwidth 0.5 absolute
set style fill solid 0.1250000 border
#set size square 1.2, 1.6
set xlabel "Iteration, i" 0,0.5  
set ylabel "E_i-E_{opt} (hartree)"  0.5,0

set logscale y
#set logscale x
 
set xrange [0:23]

#21   -3581.29270946
#24   -3581.29260656

plot       'U321GKK.dat' using ($1):($2+895.326424)/2:1   title "GAUSSIAN" with boxes, \
           'U321G.dat' using ($1):(($2+3581.29260656)/8  ) title "QUICCA" with lp ls 1

set output "UREA_STO3G.eps"
set xrange [0:18]

plot       'USTOC98.dat' using ($1):($2+442.084595):1   title "CRYSTAL" with boxes, \
           'USTO3G.dat' using ($1):(($2+3536.67736828)/8  ) title "QUICCA" with lp ls 1

#     19        -3536.67736828

# C98:
#-442.069367
#-442.084595
